Denoising Score Matching with Random Features: Insights on Diffusion Models from Precise Learning Curves

We theoretically investigate the phenomena of generalization and memorization in diffusion models. Empirical studies suggest that these phenomena are influenced by model complexity and the size of the training dataset. In our experiments, we further observe that the number of noise samples per data sample ($m$) used during Denoising Score Matching (DSM) plays a significant and non-trivial role. We capture these behaviors and shed insights into their mechanisms by deriving asymptotically precise expressions for test and train errors of DSM under a simple theoretical setting. The score function is parameterized by random features neural networks, with the target distribution being $d$-dimensional Gaussian. We operate in a regime where the dimension $d$, number of data samples $n$, and number of features $p$ tend to infinity while keeping the ratios $\psi_n=\frac{n}{d}$ and $\psi_p=\frac{p}{d}$ fixed. By characterizing the test and train errors, we identify regimes of generalization and memorization as a function of $\psi_n,\psi_p$, and $m$. Our theoretical findings are consistent with the empirical observations.

==> sections/denoiser.tex <==
\section{Test and train error when learning denoiser}

\subsection{Random Features model}
In this section, we assume $s_\theta(t,x)=\rat{A_t}{p}\varrho(\rat{W_t}{d}x)$, $W_t\in\R^{p\times d}$, $A_t\in\R^{d\times p}$, where the elements of $W_t$ are distributed as $\cN{0,1}$, and $x_i\sim\pi\equiv\cN{0,I_d}$, $z_{ij}\sim\cN{0,I_d}$.
\begin{align*}
    \hat{\cL}_t(A_t) &= \frac{1}{nm}\sum_{i=1}^{n}{\sum_{j=1}^{m}\norm{\rat{A_t}{p}\varrho(\rat{W_t}{d}(a_tx_i+\sqrt{h_t}z_{ij})-x_i}^2}+\frac{\lambda}{p}\norm{A_t}_F^2,\\
    &= \frac{1}{nm}\sum_{i=1}^{n}{\norm{\rat{A_t}{p}\varrho(\rat{W_t}{d}(a_tx_i\textbf{1}^T+\sqrt{h_t}Z_i)-x_i\textbf{1}^T}_F^2}+\frac{\lambda}{p}\norm{A_t}_F^2,\\
    &=\textbf{tr}\{\rat{A_t^T}{p}\rat{A_t}{p} (U+\lambda I_p)\}-2\textbf{tr}\{\rat{A_t}{p} V\}+d,\\
\end{align*}
where $Z_i = [z_{i1},z_{i2},\cdots,z_{im}]$,
$$U = \frac{1}{nm}\sum_{i=1}^n{\varrho(\rat{W_t}{d}(a_tx_i\textbf{1}^T+\sqrt{h_t}Z_i))\varrho(\rat{W_t}{d}(a_tx_i\textbf{1}^T+\sqrt{h_t}Z_i))^T}$$ and 
$$V = \frac{1}{nm}\sum_{i=1}^n{\varrho(\rat{W_t}{d}(a_tx_i\textbf{1}^T+\sqrt{h_t}Z_i))(x_i\textbf{1}^T)^T}.$$
Thus we get the optimal $A_t$ as
\begin{equation}
    \rat{\hat{A}_t}{p} = V^T (U+\lambda I_p)^{-1}.
\end{equation}
We now consider two extreme cases: when $m=1$ and $m=\infty$.\\
\subsubsection{Case: $m=\infty$}
When $m=\infty$, the loss function reduces as follows:
\begin{align}
    \cL_t(s) &= \frac{1}{n}\sum_{i=1}^{n}{\bE{z\sim\cN{0,I_d}}{\norm{s(t,a_tx_i+\sqrt{h_t}z)-x_i}^2}}.
\end{align}
We have $s_\theta(t,x)=\rat{A_t}{p}\varrho(\rat{W_t}{d}x)$, $W_t\in\R^{p\times d}$, $A_t\in\R^{d\times p}$.
\begin{align*}
    \cL_t(A_t) &=\frac{1}{n}\sum_{i=1}^{n}{\bE{z}{\norm{\rat{A_t}{p}\varrho(\rat{W_t}{p}(a_tx_i+\sqrt{h_t}z))-x_i}^2}}+\frac{\lambda}{p}\norm{A_t}_F^2,\\
    &=\tr{\rat{A_t}{p}^T\rat{A_t}{p} U}-2\tr{\rat{A_t}{p} V}+d+\lambda\tr{\rat{A_t^T}{p}\rat{A_t}{p}},\\
\end{align*}
where 
$$U = \frac{1}{n}\sum_{i=1}^n\bE{z}{\varrho(\rat{W_t}{d}(a_tx_i+\sqrt{h_t}z))\varrho(\rat{W_t}{d}(a_tx_i+\sqrt{h_t}z))^T}$$
and 
$$V = \frac{1}{n}\sum_{i=1}^n\bE{z}{\varrho(\rat{W_t}{d}(a_tx_i+\sqrt{h_t}z))x_i^T}.$$ Thus we get the optimal $A_t$ as
\begin{equation}
    \rat{\hat{A}_t}{p} = V^T(U+\lambda I_p)^{-1}.
\end{equation}
Now, we compute test error (generalization error) and train error when $\pi\equiv\cN{0,I_d}$. We note that $P_t\equiv\cN{0,1}$.\\
\textbf{Test Error:}
\begin{align*}
    \cE_{\text{test}} &= \frac{1}{d}\bE{x\sim P_t}{\norm{\rat{\hat{A}_t}{p}\varrho(\rat{W_t}{d}x)-ax}^2}\\
    &=a^2 - \frac{2a}{d}\tr{V^T (U+\lambda I_p)^{-1}\underbrace{\bE{x}{\varrho(\rat{W_t}{d}x)x^T}}_{:=\Tilde{V}}}\\
    &\qquad+\frac{1}{d}\tr{(U+\lambda I_p)^{-1}V V^T(U+\lambda I_p)^{-1}\underbrace{\bE{x}{\varrho(\rat{W_t}{d}x)\varrho(\rat{W_t}{d}x)^T}}_{:=\Tilde{U}}}
\end{align*}
Since we focus on a single time instant, we drop the subscript $t$ in the above expressions. However, we will keep in mind that $a$ and $h$ depend on $t$ and we have the relation $a^2+h=1$.

We need to compute $V,U,\Tilde{V},\Tilde{U}$ in order to get an expression for $\cE_{\text{test}}$. We will first consider $\Tilde{V}$.

\begin{equation*}
    \Tilde{V} = \bE{x}{\varrho(\rat{W}{d}x)x^T}
\end{equation*}
Let $w_i$ denote the $i^{\text{th}}$ row of $W$. Let $P_\gamma$ denote the bivariate standard Gaussian distribution with correlation coefficient $\gamma$. We have 
\begin{align*}
    \Tilde{V}_{ij} &= \bE{x}{\varrho(\rat{w_i^Tx}{d})x_j}\\
    &= \bE{(u,v)\sim P_{\rat{w_{ij}}{d}}}{\varrho(u)v}\\
    &\stackrel{(a)}{=} \sum_{k=0}^{\infty} \frac{(\rat{w_{ij}}{d})^k}{k!}\bE{u}{\varrho(u)\text{He}_k(u)}\bE{v}{v\text{He}_k(v)}\\
    &= \mu_1\rat{w_{ij}}{d},
\end{align*}
where in $(a)$ we used the Mehler Kernel formula.
Hence, we have $\Tilde{V} = \mu_1\rat{W}{d}$. Now, we consider $\Tilde{U}$.
\begin{align*}
    \Tilde{U}_{ij} &= \bE{x}{\varrho(\rat{w_i^Tx}{d})\varrho(\rat{w_j^Tx}{d})}\\
    &= \bE{(u,v)\sim P_{\frac{w_i^Tw_j}{d}}}{\varrho(u)\varrho(v)}\\
    &= \sum_{k=0}^{\infty} \frac{(\frac{w_i^Tw_j}{d})^k}{k!}\bE{u}{\varrho(u)\text{He}_k(u)}\bE{u}{\varrho(v)\text{He}_k(v)}\\
    &= \sum_{k=0}^{\infty} \frac{(\frac{w_i^Tw_j}{d})^k}{k!}\bE{u}{\varrho(u)\text{He}_k(u)}^2.
\end{align*}
Let $\mu_0 = \bE{g}{\varrho(g)}, \mu_1 = \bE{g}{\varrho(g)g}, \norm{\varrho}^2 = \bE{g}{\varrho(g)^2}$. Then, we have
\begin{equation*}
    \Tilde{U}_{ij} = \begin{cases}
        \mu_0^2+\mu_1^2 \frac{w_i^Tw_j}{d} + O(1/d)\quad &\text{if } i\neq j,\\
        \norm{\varrho}^2\quad &\text{if } i=j.
    \end{cases}
\end{equation*}
Let $v^2 = \norm{\rho}^2-\mu_0^2-\mu_1^2$. Neglecting $O(1/d)$ terms, we have
\begin{equation*}
    \Tilde{U} = \mu_0^2 \bone\bone^T + \mu_1^2 \rat{W}{d}\rat{W^T}{d} + v^2 I_p
\end{equation*}
Now we will consider $V$. Let
\begin{equation*}
    V^l = \bE{z}{\varrho(\rat{W}{d}(ax_l+\sqrt{h}z))x_l^T}
\end{equation*}
We have 
\begin{align*}
    V^l_{ij} &= \bE{z}{\varrho(\rat{w_i^T(ax_l+\sqrt{h}z)}{d})x_{lj}}\\
    &= \bE{u}{\varrho(\rat{a w_i^Tx_l}{d}+\sqrt{h}u)}x_{lj}\\
    &= \varrho_0(\rat{a w_i^Tx_l}{d})x_{lj}.
\end{align*}
where $\varrho_0(y) = \bE{u}{\varrho(y+\sqrt{h}u)}$.
\begin{align*}
    V_{ij} &= \frac{1}{n}\sum_{l=1}^{n} V^l_{ij},\\
    &= \frac{1}{n}\sum_{l=1}^{n} \varrho_0(\rat{a w_i^Tx_l}{d})x_{lj},\\
\end{align*}
We have $V = \rat{\varrho_0(a\rat{W}{d}X)}{n}\rat{X^T}{n}$. Now, let's consider $U$. Let
\begin{align*}
    U^l &= \bE{z}{\varrho(\rat{W}{d}(ax_l+\sqrt{h}z))\varrho(\rat{W}{d}(ax_l+\sqrt{h}z))^T}\\
\end{align*}
For $i\neq j $ we have,
\begin{align*}
    U^l_{ij} &= \bE{z}{\varrho(\rat{w_i^T(ax_l+\sqrt{h}z)}{d})\varrho(\rat{w_j^T(ax_l+\sqrt{h}z)}{d})}\\
    &= \bE{(u,v)\sim P_{\frac{w_i^Tw_j}{d}}}{\varrho(a\rat{w_i^Tx_l}{d} + \sqrt{h}u)\varrho(a\rat{w_j^Tx_l}{d} + \sqrt{h}v)}\\
    &= \sum_{k=0}^{\infty} \frac{(\frac{w_i^Tw_j}{d})^k}{k!}\bE{u}{\varrho(a\rat{w_i^Tx_l}{d} + \sqrt{h}u)\text{He}_k(u)}\bE{u}{\varrho(a\rat{w_j^Tx_l}{d} + \sqrt{h}v)\text{He}_k(v)}\\
    &= \varrho_0(a\rat{w_i^Tx_l}{d})\varrho_0(a\rat{w_j^Tx_l}{d})+\frac{w_i^Tw_j}{d}\varrho_1(a\rat{w_i^Tx_l}{d})\varrho_1(a\rat{w_j^Tx_l}{d})+O(1/d),
\end{align*}
where $\varrho_0(y) = \bE{u}{\varrho(y+\sqrt{h}u)}$ and $\varrho_1(y) = \bE{u}{\varrho(y+\sqrt{h}u)u}$. Let $X=[x_1, x_2,\cdots,x_n]\in\R^{d\times n}$. 
\begin{align*}
    U_{ij} &= \frac{1}{n}\sum_{l=1}^{n} U^l_{ij},\\
    &= \frac{1}{n}\sum_{l=1}^{n}\varrho_0(a\rat{w_i^Tx_l}{d})\varrho_0(a\rat{w_j^Tx_l}{d})+\frac{w_i^Tw_j}{d}\frac{1}{n}\sum_{l=1}^{n}\varrho_1(a\rat{w_i^Tx_l}{d})\varrho_1(a\rat{w_j^Tx_l}{d}) + O(1/d)\\
    &= \frac{1}{n}\sum_{l=1}^{n}\varrho_0(a\rat{w_i^Tx_l}{d})\varrho_0(a\rat{w_j^Tx_l}{d})+\frac{w_i^Tw_j}{d}\bE{x}{\varrho_1(a\rat{w_i^Tx}{d})\varrho_1(a\rat{w_j^Tx}{d})} + O(1/d)\\
    &= \frac{1}{n}\sum_{l=1}^{n}\varrho_0(a\rat{w_i^Tx_l}{d})\varrho_0(a\rat{w_j^Tx_l}{d})+\frac{w_i^Tw_j}{d}\bE{g}{\varrho_1(ag)}^2 + O(1/d)\\
    &= \frac{1}{n}\sum_{l=1}^{n}\varrho_0(a\rat{w_i^Tx_l}{d})\varrho_0(a\rat{w_j^Tx_l}{d})+h\mu_1^2\frac{w_i^Tw_j}{d} + O(1/d)\\
\end{align*}
For $i=j$,
\begin{align*}
    U^l_{ii} &= \bE{z}{\left(\varrho(\rat{w_i^T(ax_l+\sqrt{h}z)}{d})\right)^2}\\
\end{align*}
\begin{align*}
    U_{ii} &= \frac{1}{n}\sum_{l=1}^n\bE{z}{\left(\varrho(\rat{w_i^T(ax_l+\sqrt{h}z)}{d})\right)^2}\\
    &= \bE{z,x}{\left(\varrho(\rat{w_i^T(ax_l+\sqrt{h}z)}{d})\right)^2}+O(1/\sqrt{d})\\
    &= \norm{\varrho}^2+O(1/\sqrt{d}).
\end{align*}
Let $X=[x_1,x_2,\cdots,x_n]$. We can write $U$ as:
\begin{equation*}
    U = \rat{\varrho_0(a\rat{W}{d}X)}{n}\rat{\varrho_0(a\rat{W}{d}X)^T}{n}+h\mu_1^2\rat{W}{d}\rat{W^T}{d}+s^2I_p,
\end{equation*}
where
\begin{align*}
s^2 &= \norm{\varrho}^2-\bE{g}{\varrho_0(ag)^2}-h\mu_1^2\\
&= \norm{\varrho}^2-\bE{g}{\bE{u}{\varrho(ag+\sqrt{h}u)}^2}-h\mu_1^2\\
&= \norm{\varrho}^2-c(a^2)-h\mu_1^2,
\end{align*}
where $c(\gamma) = \bE{u,v\sim P_\gamma}{\varrho(u)\varrho(v)}$.

We can use Gaussian equivalence principle to replace the nonlinear term in $U$. A Gaussian equivalent for $\varrho_0(a\rat{W}{d}X)$ is given by
\begin{align*}
    G &= \bE{g}{\varrho_0(ag)}\bone\bone^T+\bE{g}{\varrho_0(ag)g}\rat{W}{d}X+\left(\bE{g}{\varrho_0(ag)^2}-\bE{g}{\varrho_0(ag)}^2-\bE{g}{\varrho_0(ag)g}^2\right)^{1/2}\Omega\\
    &= \mu_0\bone\bone^T+a\mu_1\rat{W}{d}X+\left(\underbrace{c(a^2)-\mu_0^2-a^2\mu_1^2}_{:=v_0^2}\right)^{1/2}\Omega,
\end{align*}
where, $\Omega\in\R^{p\times n}$ is a random matrix with standard Gaussian entries.
Hence we have
\begin{align*}
    U &= \rat{G}{n}\rat{G^T}{n}+h\mu_1^2\rat{W}{d}\rat{W^T}{d}+s^2I_p,\\
    V &= \rat{G}{n}\rat{X^T}{n}
\end{align*}
where,
\begin{equation*}
    G = \mu_0\bone\bone^T+a\mu_1\rat{W}{d}X+v_0\Omega.
\end{equation*}
We now have expressions for all terms in the generalization error.
\begin{align*}
    \cE_{\text{test}} &=a^2 - \frac{2a}{d}\tr{V^T (U+\lambda I_p)^{-1}\Tilde{V}}+\frac{1}{d}\tr{(U+\lambda I_p)^{-1}V V^T(U+\lambda I_p)^{-1}\Tilde{U}}\\
    &= a^2-\frac{2a\mu_1}{d}\tr{\rat{X}{n}\rat{G^T}{n}(U+\lambda I_p)^{-1}\rat{W}{d}}\\&\qquad+\frac{1}{d}\tr{(U+\lambda I_p)^{-1}\rat{G}{n}\rat{X^T}{n}\rat{X}{n}\rat{G^T}{n}(U+\lambda I_p)^{-1}\left(\mu_0^2 \bone\bone^T + \mu_1^2 \rat{W}{d}\rat{W^T}{d} + v^2 I_p\right)}
\end{align*}
For simplicity in presentation, assume that $\mu_0=0$.
\begin{align*}
    \cE_{\text{test}} &= a^2-2a\mu_1E_1+\mu_1^2E_2+v^2E_3.
\end{align*}
\begin{align*}
    E_1 &= \frac{1}{d}\tr{\rat{X}{n}\rat{G^T}{n}(U+\lambda I_p)^{-1}\rat{W}{d}}\\
    E_2 &= \frac{1}{d}\tr{\rat{W^T}{d}(U+\lambda I_p)^{-1}\rat{G}{n}\rat{X^T}{n}\rat{X}{n}\rat{G^T}{n}(U+\lambda I_p)^{-1}\rat{W}{d}}\\
    E_3 &= \frac{1}{d}\tr{(U+\lambda I_p)^{-2}\rat{G}{n}\rat{X^T}{n}\rat{X}{n}\rat{G^T}{n}}
\end{align*}
We define the following matrix
\begin{equation*}
    U(q) :=  \rat{G}{n}\rat{G^T}{n}+(h\mu_1^2+q)\rat{W}{d}\rat{W^T}{d}+s^2I_p,
\end{equation*}
and define the resolvent of $U(q)$ as
\begin{equation*}
    R(q,z) = (U(q)-zI_p)^{-1}.
\end{equation*}
Let 
\begin{equation*}
    K(q,z) = \frac{1}{d}\tr{R(q,z)\rat{G}{n}\rat{X^T}{n}\rat{X}{n}\rat{G^T}{n}}
\end{equation*}
Using the identities $\frac{\partial R}{\partial q} = -R(q,z)\frac{\dd U}{\dd q}R(q,z)$ and $\frac{\partial R}{\partial z} = R(q,z)^2$, we observe that 
\begin{align*}
    % E_1 &= K(0,-\lambda)\\
    E_2 &= -\frac{\partial K}{\partial q}(0,-\lambda)\\
    E_3 &= \frac{\partial K}{\partial z}(0,-\lambda)
\end{align*}
Therefore, it suffices to have the function $K$ and $E_1$ to have an expression for $\cE_{\text{test}}$.
We derive an expression for $K$ and $E_1$ using Linear pencils. We construct the following $4\times 4$ block matrix.
\begin{equation*}
    L = \mleft[
        \begin{array}{c|ccc}
        (s^2-z)I_p & a\mu_1\rat{W}{d} & v_0\rat{\Omega}{n} & (h\mu_1^2+q)\rat{W}{d}\\
        \hline
        0 & I_d & -\rat{X}{n} & 0\\
        -v_0\rat{\Omega^T}{n} & 0 & I_n & -a\mu_1\rat{X^T}{n}\\
        -\rat{W^T}{d} & 0 & 0 & I_d
    \end{array}
    \mright] = \mleft[\begin{array}{cc}
        L_{11} & L_{12} \\
        L_{21} & L_{22}
    \end{array}\mright].
\end{equation*}
First, we can invert $L$ and verify that $K$ is trace of one of the blocks in $L^{-1}$. Let $\bar{L}_{22} = L_{11}-L_{12}L_{22}^{-1}L_{21}$. Using Block matrix inversion formula, we have 
\begin{equation*}
    L^{-1} = \mleft[
            \begin{array}{cc}
              \bar{L}_{22}^{-1}   &  -\bar{L}_{22}^{-1}L_{12}L_{22}^{-1}\\
               -L_{22}^{-1}L_{21}\bar{L}_{22}^{-1}  &  L_{22}^{-1}+ L_{22}^{-1}L_{21}\bar{L}_{22}^{-1}L_{12}L_{22}^{-1}
            \end{array}
    \mright]
\end{equation*}.
\begin{equation*}
    L_{22}^{-1} = \mleft[\begin{array}{ccc}
       I_d  &  \rat{X}{n} & a\mu_1\rat{X}{n}\rat{X^T}{n}\\
       0  & I_n & a\mu_1\rat{X^T}{n}\\
       0  & 0 & I_d\\
    \end{array}\mright]
\end{equation*}
\begin{align*}
    \bar{L}_{22} &= (s^2-z)I_p + v_0\rat{G}{n}\rat{\Omega^T}{n}+a\mu_1\rat{G}{n}\rat{X^T}{n}\rat{W^T}{d}+(h\mu_1^2+q)\rat{W}{d}\rat{W^T}{d}\\
    &= (s^2-z)I_p + \rat{G}{n}\rat{G^T}{n}+(h\mu_1^2+q)\rat{W}{d}\rat{W^T}{d}\\
    &= R^{-1}(q,z)    
\end{align*}
Hence,
\begin{equation*}
\footnotesize
    L^{-1} = \mleft[
    \begin{array}{cccc}
       R(q,z)  & -a\mu_1R(q,z)\rat{W}{d} & -R(q,z)\rat{G}{n} & -R(q,z)(a\mu_1\rat{G}{n}\rat{X^T}{n}+(h\mu_1^2+q)\rat{W}{d}) \\
        \rat{X}{n}\rat{G^T}{n}R(q,z) & I_d-a\mu_1\rat{X}{n}\rat{G^T}{n}R(q,z)\rat{W}{d} & \rat{X}{n}-\rat{X}{n}\rat{G^T}{n}R(q,z)\rat{G}{n} & a\mu_1\rat{X}{n}\rat{X^T}{n}-\rat{X}{n}\rat{G^T}{n}R(q,z)(a\mu_1\rat{G}{n}\rat{X^T}{n}+(h\mu_1^2+q)\rat{W}{d})\\
        \rat{G^T}{n}R(q,z) & -a\mu_1\rat{G^T}{n}R(q,z)\rat{W}{d} & I_n-\rat{G^T}{n}R(q,z)\rat{G}{n} & a\mu_1\rat{X^T}{n}-\rat{G^T}{n}R(q,z)(a\mu_1\rat{G}{n}\rat{X^T}{n}+(h\mu_1^2+q)\rat{W}{d})\\
        \rat{W^T}{d} & -a\mu_1\rat{W^T}{d}R(q,z)\rat{W}{d} & -\rat{W^T}{d}R(q,z)\rat{G}{n} & I_d-\rat{W^T}{d}R(q,z)(a\mu_1\rat{G}{n}\rat{X^T}{n}+(h\mu_1^2+q)\rat{W}{d})
    \end{array}
    \mright]
\end{equation*}
We see that $(L^{-1})^{2,2}$ and $(L^{-1})^{2,4}$ give the desired terms. We have
\begin{align*}
    \frac{1}{d}\tr{(L^{-1})^{2,2}} &= 1-a\mu_1E_1\\ 
    \frac{1}{d}\tr{(L^{-1})^{2,4}} &= a\mu_1-a\mu_1K(q,z)-(h\mu_1^2+q)E_1\\ 
\end{align*}
We use the linear pencil formalism to derive the traces of of square blocks in $L^{-1}$. Let $g$ be the matrix of traces of square blocks in $L^{-1}$ divided by the block size. For example, if $L^{i,j}$ is a square matrix of dimension $N$, then $g_{ij}=\frac{1}{N}\tr{(L^{-1})^{i,j}}$. We assign $g_{ij}=0$ if $L^{i,j}$ is not a square matrix.
\begin{equation*}
    g = \mleft[
    \begin{array}{cccc}
        g_{11} & 0 & 0 & 0  \\
        0 & g_{22} & 0 & g_{24}  \\
        0 & 0 & g_{33} & 0  \\
        0 & g_{42} & 0 & g_{44}  \\
    \end{array}
    \mright]
\end{equation*}
Notice that the constant matrices in $L$ are all multiples of identity. Let $B$ be the matrix that contains the coefficients of these constant matrices.
\begin{equation*}
    B = \mleft[
    \begin{array}{cccc}
        s^2-z & 0 & 0 & 0  \\
        0 & 1 & 0 & 0  \\
        0 & 0 & 1 & 0  \\
        0 & 0 & 0 & 1  \\
    \end{array}
    \mright]
\end{equation*}
If $L^{il}$ and $L^{jk}$ are square matrices, let $\sigma_{ij}^{kl}$ be the covariance between an element of $L^{ij}$ and $L^{kl}$ multiplied by the block size of $L^{jk}$. Let $L^{ij}$ be of dimension $N_i\times N_j$ and $M$ denote the non constant part of $L$. Then,
\begin{equation*}
    \sigma_{ij}^{kl} = N_j\bE{}{M^{ij}_{uv}M^{kl}_{vu}}.
\end{equation*}
Let $S = \{(i,j): N_i=N_j\}$, the set of indices of square blocks in $L$. Then, a mapping $\eta_L$ is defined such that
\begin{equation*}
    \eta_L(G)_{il} = \sum_{(jk) \in S} \sigma_{ij}^{kl}g_{jk}
\end{equation*}
for $(il)$ in $S$. 
\begin{equation*}
    \eta_L(g) = \mleft[
    \begin{array}{cccc}
        \sigma_{12}^{41}g_{24}+\sigma_{13}^{31}g_{33}+\sigma_{14}^{41}g_{44} & 0 & 0 & 0  \\
        0 & 0 & 0 & \sigma_{23}^{34}g_{33}  \\
        0 & 0 & \sigma_{31}^{13}g_{11}+\sigma_{34}^{23}g_{42} & 0  \\
        0 & \sigma_{41}^{12}g_{11} & 0 & \sigma_{41}^{14}g_{11}  \\
    \end{array}
    \mright]
\end{equation*}
We have $N_1=p, N_2=d, N_3=n, N_4=d$.
\begin{align}
    & \sigma_{12}^{41} = -a\mu_1,\qquad \sigma_{41}^{12}= -a\mu_1\psi_p\\
    & \sigma_{13}^{31} = -v_0^2,\qquad \sigma_{31}^{13} = -v_0^2\psi_p/\psi_n\\
    & \sigma_{14}^{41} = -(h\mu_1^2+q),\qquad \sigma_{41}^{14} = -(h\mu_1^2+q)\psi_p\\
    & \sigma_{23}^{34} = a\mu_1,\qquad \sigma_{34}^{23}=a\mu_1/\psi_n\\
\end{align}
We have that $g$ satisfies the following fixed point equation
\begin{equation*}
    (B-\eta_L(g))g = I.
\end{equation*}
Hence we have,
\begin{multline*}
    \mleft[
    \begin{array}{cccc}
        s^2-z+a\mu_1g_{24}+v_0^2g_{33}+(h\mu_1^2+q)g_{44} & 0 & 0 & 0  \\
        0 & 1 & 0 & -a\mu_1g_{33}  \\
        0 & 0 & 1+v_0^2\psi_p/\psi_ng_{11}-a\mu_1/\psi_ng_{42} & 0  \\
        0 & a\mu_1\psi_pg_{11} & 0 & 1+(h\mu_1^2+q)\psi_pg_{11}  \\
    \end{array}
    \mright]\\
    \times
    \mleft[
    \begin{array}{cccc}
        g_{11} & 0 & 0 & 0  \\
        0 & g_{22} & 0 & g_{24}  \\
        0 & 0 & g_{33} & 0  \\
        0 & g_{42} & 0 & g_{44}  \\
    \end{array}
    \mright] = I
\end{multline*}
This gives the following set of equations:
\begin{align*}
    g_{11}(s^2-z+a\mu_1g_{24}+v_0^2g_{33}+(h\mu_1^2+q)g_{44}) &= 1\\
    g_{22} -a\mu_1g_{33}g_{42} &= 1\\
    g_{24} -a\mu_1g_{33}g_{44} &= 0\\
    g_{33}(1+v_0^2\psi_p/\psi_ng_{11}-a\mu_1/\psi_ng_{42}) &=1\\
    a\mu_1\psi_pg_{11}g_{22}+(1+(h\mu_1^2+q)\psi_pg_{11})g_{42} &= 0\\
    a\mu_1\psi_pg_{11}g_{24}+(1+(h\mu_1^2+q)\psi_pg_{11})g_{44} &= 1\\
\end{align*}
We solve the above set of equations numerically to obtain the elements of matrix $g$. We obtain $E_1, K$ using the expressions $E_1 = \frac{1-g_{22}}{a\mu_1}$, $K(q,z)=\frac{a\mu_1-g_{24}-(h\mu_1^2+q)E_1}{a\mu_1}$. Figs.~\ref{fig:rfm_minf_test_train_err} and \ref{fig:rfm_minf_test_train_err_time} shows the test error thus obtained. Next, we look at the train error:\\
\textbf{Train error:}
\begin{align*}
    \cE_{\text{train}} &= \frac{1}{d}\cL(\hat{A})\\
    &=\frac{1}{d}\tr{\rat{\hat{A}_t}{p}^T\rat{\hat{A}_t}{p} (U+\lambda I_p)}-\frac{2}{d}\tr{\rat{\hat{A}_t}{p} V}+1,\\
    &=\frac{1}{d}\tr{(U+\lambda I_p)^{-1}VV^T}-\frac{2}{d}\tr{V^T(U+\lambda I_p)^{-1}V}+1,\\
    &=-\frac{1}{d}\tr{(U+\lambda I_p)^{-1}\rat{G}{n}\rat{X^T}{n}\rat{X}{n}\rat{G^T}{n}}+1,\\
    &=-K(0,-\lambda)+1,\\
\end{align*}
Figs.~\ref{fig:rfm_minf_test_train_err} and \ref{fig:rfm_minf_test_train_err_time} shows the train error.
\begin{figure}
    \centering
\includegraphics[width=1\linewidth]{figures/lp_minf_err.png}
    \caption{Test error and train error for $m=\infty$ case.}
    \label{fig:rfm_minf_test_train_err}
\end{figure}

\begin{figure}
    \centering
\includegraphics[width=1\linewidth]{figures/lp_err_minf_time.png}
    \caption{Test error and train error for $m=\infty$ case.}
    \label{fig:rfm_minf_test_train_err_time}
\end{figure}
\subsubsection{Case: $m=1$}
When $m=1$, the loss function reduces to:
\begin{align}
    \cL_t(s) &= \frac{1}{n}\sum_{i=1}^{n}{\norm{s(t,a_tx_i+\sqrt{h_t}z_i)-x_i}^2}.
\end{align}

Let $s_\theta(t,x)=\rat{A_t}{p}\varrho(\rat{W_t}{d}x)$, $W_t\in\R^{p\times d}$, $A_t\in\R^{d\times p}$, $X=[x_1,x_2,\cdots,x_n]$, $Z=[z_1,z_2,\cdots,z_n]$, and let $Y$ be a matrix with its $i^{th}$ column given as $y_i = a_tx_i+\sqrt{h_t}z_i$. Let $F=\varrho(\rat{W}{d}Y)$.
\begin{align*}
    \cL_t(A_t) &=\frac{1}{n}\sum_{i=1}^{n}{{\norm{\rat{A_t}{p}\varrho(\rat{W_t}{p}(a_tx_i+\sqrt{h_t}z_i))-x_i}^2}}+\frac{\lambda}{p}\norm{A_t}_F^2,\\
    &=\tr{\rat{A_t}{p}^T\rat{A_t}{p} U}-2\tr{\rat{A_t}{p} V}+d+\lambda\tr{\rat{A_t^T}{p}\rat{A_t}{p}},\\
\end{align*}
where 
$$U = \frac{1}{n}\varrho(\rat{W_t}{d}Y)\varrho(\rat{W_t}{d}Y)^T = \rat{F}{n}\rat{F^T}{n}$$
and 
$$V = \frac{1}{n}{\varrho(\rat{W_t}{d}Y)Z^T} = \rat{F}{n}\rat{X^T}{n}.$$ Thus we get the optimal $A_t$ as
\begin{equation}
    \rat{\hat{A}_t}{p} = V^T(U+\lambda I_p)^{-1} = \rat{X}{n}\rat{F^T}{n}\left(\rat{F}{n}\rat{F^T}{n}+\lambda I_p\right)^{-1}.
\end{equation}
\textbf{Test error:}
\begin{align*}
    \cE_{\text{test}} &= \frac{1}{d}\bE{x\sim P_t}{\norm{\rat{\hat{A}_t}{p}\varrho(\rat{W_t}{d}x)-ax}^2}\\
    &=a^2 - \frac{2a}{d}\tr{\rat{\hat{A}_t}{p}\underbrace{\bE{x}{\varrho(\rat{W_t}{d}x)x^T}}_{:=\Tilde{V}}}\\
    &\qquad+\frac{1}{d}\tr{\rat{\hat{A}^T_t}{p}\rat{\hat{A}_t}{p}\underbrace{\bE{x}{\varrho(\rat{W_t}{d}x)\varrho(\rat{W_t}{d}x)^T}}_{:=\Tilde{U}}}
\end{align*}

We have already derived expressions for $\Tilde{V}$ and $\Tilde{U}$ in the previous section. We have $\Tilde{V} = \mu_1\rat{W}{d}$, $\Tilde{U} = \mu_0^2\textbf{1}\textbf{1}^T+ \mu_1^2\rat{W}{d}\rat{W^T}{d}+v^2I_p$. For simplicity, we will assume that $\mu_0=0$. Thus we have

\begin{align*}
    \cE_{\text{test}} &= \frac{1}{d}\bE{x\sim P_t}{\norm{\rat{\hat{A}_t}{p}\varrho(\rat{W_t}{d}x)-ax}^2}\\
    &=a^2 - \frac{2a\mu_1}{d}\tr{\rat{X}{n}\rat{F^T}{n}\left(\rat{F}{n}\rat{F^T}{n}+\lambda I_p\right)^{-1}\rat{W}{d}}\\
    &\qquad+\frac{\mu_1^2}{d}\tr{\left(\rat{F}{n}\rat{F^T}{n}+\lambda I_p\right)^{-1}\rat{F}{n}\rat{X^T}{n}\rat{X}{n}\rat{F^T}{n}\left(\rat{F}{n}\rat{F^T}{n}+\lambda I_p\right)^{-1}\rat{W}{d}\rat{W^T}{d}}\\
    &\qquad+\frac{v^2}{d}\tr{\left(\rat{F}{n}\rat{F^T}{n}+\lambda I_p\right)^{-1}\rat{F}{n}\rat{X^T}{n}\rat{X}{n}\rat{F^T}{n}\left(\rat{F}{n}\rat{F^T}{n}+\lambda I_p\right)^{-1}}
\end{align*}
Since we focus on a single time instant, we drop the subscript $t$ in the above expressions. However, we will keep in mind that $a$ and $h$ depend on $t$ and we have the relation $a^2+h=1$. Also, we use Gaussian equivalence principle to handle the non-linearity in $F$. In particular, we use the following expression for $F$:
\begin{equation*}
    F = \mu_1\rat{W}{d}Y+v\Omega.
\end{equation*}
Let 
\begin{equation}
    R(q,z) = \left(\rat{F}{n}\rat{F^T}{n}+q\rat{W}{d}\rat{W^T}{d}-zI_p\right)^{-1},
\end{equation}
and
\begin{align*}
    E_1 &= \frac{1}{d}\tr{\rat{X}{n}\rat{F^T}{n}R(0,-\lambda)\rat{W}{d}}\\
    E_2 &= \frac{1}{d}\tr{R(0,-\lambda)\rat{F}{n}\rat{X^T}{n}\rat{X}{n}\rat{F^T}{n}R(0,-\lambda)\rat{W}{d}\rat{W^T}{d}}\\
    E_3 &= \frac{1}{d}\tr{\rat{F}{n}\rat{X^T}{n}\rat{X}{n}\rat{F^T}{n}R(0,-\lambda)^2}
\end{align*}
With above definitions, we can write $\cE_{\text{test}}$ as 
\begin{equation*}
    \cE_{\text{test}} = a^2-2a\mu_1E_1+\mu_1^2E_2+v^2E_3.
\end{equation*}
Let 
\begin{align*}
    K(q,z) = \frac{1}{d}\tr{R(q,z)\rat{F}{n}\rat{X^T}{n}\rat{X}{n}\rat{F^T}{n}}.
\end{align*}
Then we have 
\begin{align*}
    E_2 &= -\frac{\dd K}{\dd q}(0,-\lambda)\\
    E_3 &= \frac{\dd K}{\dd z}(0,-\lambda)\\
\end{align*}
Hence, we need to find the terms $E_1$ and $K$ in order to derive an expression for the generalization error. As earlier, we use linear pencils to obtain the desired terms. We use the following $6\times 6$ linear pencil matrix for this:

\begin{equation*}
    L = \mleft[
        \begin{array}{c|ccccc}
        -zI_p & q\rat{W}{d} & v_0\rat{\Omega}{n} & \mu_1\rat{W}{d} & 0 & 0\\
        \hline
        -\rat{W^T}{d} & I_d & 0 & 0 & 0 & 0\\
        -v\rat{\Omega^T}{n} & -\mu\rat{Y^T}{n} & I_n & 0 & 0 & 0\\
        0 & 0 & -\rat{Y}{n} & I_d & 0 & 0\\
        0 & 0 & -\rat{X}{n} & 0 & I_d & 0\\
        0 & 0 & 0 & 0 & -\rat{X^T}{n} & I_n\\
    \end{array}
    \mright] = \mleft[\begin{array}{cc}
        L_{11} & L_{12} \\
        L_{21} & L_{22}
    \end{array}\mright].
\end{equation*}
By computing $L^{-1}$, we find that
\begin{align}
    (L^{-1})^{5,4}(q,z) &= -\mu_1\rat{X}{n}\rat{F^T}{n}R(q,z)\rat{W}{d}\\
    (L^{-1})^{6,3}(q,z) &= -\rat{X^T}{n}\rat{X}{n}\rat{F^T}{n}R(q,z)\rat{F}{n}+\rat{X^T}{n}\rat{X}{n}\\
\end{align}
Hence,
\begin{align}
    E_1 &= \frac{1}{d}\tr{\rat{X}{n}\rat{F^T}{n}R(0,-\lambda)\rat{W}{d}} = -\frac{1}{\mu_1 d}\tr{(L^{-1})^{5,4}(0,-\lambda)}\\
    K(q,z) &= \frac{1}{d}\tr{R(q,z)\rat{F}{n}\rat{X^T}{n}\rat{X}{n}\rat{F^T}{n}} = 1-\frac{1}{d}\tr{(L^{-1})^{6,3}(q,z)}. 
\end{align}
We can compute the traces of blocks in $L^{-1}$ as earlier. We have 
\begin{equation*}
    g = \mleft[
    \begin{array}{cccccc}
        g_{11} & 0 & 0 & 0 & 0 & 0 \\
        0 & g_{22} & 0 & g_{24} & 0 & 0 \\
        0 & 0 & g_{33} & 0 & 0 & 0 \\
        0 & g_{42} & 0 & g_{44} & 0 & 0 \\
        0 & g_{52} & 0 & g_{54} & 1 & 0 \\
        0 & 0 & g_{63} & 0 & 0 & 1  \\
    \end{array}
    \mright]
\end{equation*}

\begin{equation*}
    B = \mleft[
    \begin{array}{cccccc}
        -z & 0 & 0 & 0 & 0 & 0 \\
        0 & 1 & 0 & 0 & 0 & 0 \\
        0 & 0 & 1 & 0 & 0 & 0 \\
        0 & 0 & 0 & 1 & 0 & 0 \\
        0 & 0 & 0 & 0 & 1 & 0 \\
        0 & 0 & 0 & 0 & 0 & 1  \\
    \end{array}
    \mright]
\end{equation*}
\begin{equation*}
    \eta_L(g) = \mleft[
    \begin{array}{cccccc}
        \sigma_{12}^{21}g_{22}+\sigma_{13}^{31}g_{33}+\sigma_{14}^{21}g_{42} & 0 & 0 & 0 & 0 & 0 \\
        0 & \sigma_{21}^{12}g_{11} & 0 & \sigma_{21}^{14}g_{11} & 0 & 0 \\
        0 & 0 & \sigma_{31}^{13}g_{11}+\sigma_{32}^{43}g_{24} & 0 & 0 & 0 \\
        0 & \sigma_{43}^{32}g_{33} & 0 & 0 & 0 & 0 \\
        0 & \sigma_{53}^{32}g_{33} & 0 & 0 & 0 & 0 \\
        0 & 0 & \sigma_{65}^{43}g_{54}+\sigma_{65}^{53} & 0 & 0 & 0  \\
    \end{array}
    \mright]
\end{equation*}

\begin{align}
    & \sigma_{12}^{21} = -q,\qquad \sigma_{21}^{12}= -q\psi_p,\qquad \sigma_{21}^{14}= -\mu_1\psi_p\\
    & \sigma_{13}^{31} = -v^2,\qquad \sigma_{31}^{13} = -v^2\psi_p/\psi_n,\qquad \sigma_{32}^{43} = \mu_1/\psi_n,\qquad \sigma_{43}^{32} = \mu_1\\
    & \sigma_{14}^{21} = -\mu_1,\qquad \sigma_{53}^{32} = \mu_1a\\
    & \sigma_{65}^{43} = a/\psi_n,\qquad \sigma_{65}^{53}=1/\psi_n\\
\end{align}
We have that $g$ satisfies the following fixed point equation
\begin{equation*}
    (B-\eta_L(g))g = I.
\end{equation*}
Hence we have,
\begin{multline*}
    \mleft[
    \begin{array}{cccccc}
        -z+qg_{22}+v^2g_{33}+\mu_1g_{42} & 0 & 0 & 0 & 0 & 0  \\
        0 & 1+q\psi_p g_{11} & 0 & \mu_1\psi_p g_{11} & 0 & 0  \\
        0 & 0 & 1+v^2\psi_p/\psi_ng_{11}-\mu_1/\psi_ng_{24} & 0 & 0 & 0  \\
        0 & -\mu_1g_{33} & 0 & 1 & 0 & 0  \\
        0 & -\mu_1ag_{33} & 0 & 0 & 1 & 0  \\
        0 & 0 & -a/\psi_n g_{54}-1/\psi_n & 0 & 0 & 1  \\
    \end{array}
    \mright]\\
    \times
    \mleft[
    \begin{array}{cccccc}
        g_{11} & 0 & 0 & 0 & 0 & 0 \\
        0 & g_{22} & 0 & g_{24} & 0 & 0 \\
        0 & 0 & g_{33} & 0 & 0 & 0 \\
        0 & g_{42} & 0 & g_{44} & 0 & 0 \\
        0 & g_{52} & 0 & g_{54} & 1 & 0 \\
        0 & 0 & g_{63} & 0 & 0 & 1  \\
    \end{array}
    \mright] = I
\end{multline*}
This gives the following set of equations:
\begin{align*}
    g_{11}(-z+qg_{22}+v^2g_{33}+\mu_1g_{42}) &= 1\\
    g_{22}(1+q\psi_p g_{11}) +\mu_1\psi_pg_{11}g_{42} &= 1\\
    g_{24}(1+q\psi_p g_{11}) +\mu_1\psi_pg_{11}g_{44} &= 0\\
    g_{33}(1+v^2\psi_p/\psi_ng_{11}-\mu_1/\psi_ng_{24}) &= 1\\
    -\mu_1g_{22}g_{33}+g_{42} &= 0\\
    -\mu_1g_{24}g_{33}+g_{44} &= 1\\
    -\mu_1ag_{33}g_{22}+g_{52} &= 0\\
    -\mu_1ag_{33}g_{24}+g_{54} &= 0\\
    g_{33}(-a/\psi_n g_{54}-1/\psi_n)+g_{63} &= 0 
\end{align*}
As earlier, we solve the above set of equations to obtain the elements of matrix $g$. We obtain $E_1, K$ by using the expressions $E_1 = -g_{54}/\mu_1$, $K(q,z)=1-\psi_ng_{63}$. Fig.~\ref{fig:rfm_m1_test_train_err} and \ref{fig:rfm_m1_test_train_err_time} shows the test error thus obtained.\\
\textbf{Train error:}
\begin{align*}
    \cE_{\text{train}}    &=\frac{1}{d}\tr{\rat{\hat{A}_t}{p}^T\rat{\hat{A}_t}{p} (U+\lambda I_p)}+\frac{2}{\sqrt{h}d}\tr{\rat{\hat{A}_t}{p} V}+\frac{1}{h},\\
    &=\frac{1}{hd}\tr{(U+\lambda I_p)^{-1}VV^T}-\frac{2}{hd}\tr{V^T(U+\lambda I_p)^{-1}V}+\frac{1}{h},\\
    &=-\frac{1}{hd}\tr{(U+\lambda I_p)^{-1}\rat{F}{n}\rat{Z^T}{n}\rat{Z}{n}\rat{F^T}{n}}+\frac{1}{h},\\
    &=-\frac{K(0,-\lambda)}{h}+\frac{1}{h},\\
\end{align*}
Figs~\ref{fig:rfm_m1_test_train_err} and \ref{fig:rfm_m1_test_train_err_time} shows the train error.
\begin{figure}
    \centering
\includegraphics[width=1\linewidth]{figures/lp_m1_err.png}
    \caption{Test error and train error for $m=1$ case.}
    \label{fig:rfm_m1_test_train_err}
\end{figure}

\begin{figure}
    \centering
\includegraphics[width=1\linewidth]{figures/lp_err_m1_time.png}
    \caption{Test error and train error for $m=1$ case.}
    \label{fig:rfm_m1_test_train_err_time}
\end{figure}

